Phase-Field Model of Silicon Carbide Growth During Isothermal Condition

Silicon carbide (SiC) emerges as a promising ceramic material for high-temperature structural applications, especially within the aerospace sector. The utilization of SiC-based ceramic matrix composites (CMCs) instead of superalloys in components like engine shrouds, combustors, and nozzles offers notable advantages, including a 25% improvement in fuel efficiency, over 10% enhanced thrust, and the capability to withstand up to 500$^{\circ}$C higher operating temperatures. Employing a CALPHAD-reinforced multi-phase-field model, our study delves into the evolution of the SiC layer under isothermal solidification conditions. By modeling the growth of SiC between liquid Si and solid C at 1450$^{\circ}$C, we compared results with experimental microstructures and quantitatively examined the evolution of SiC thickness over time. Efficient sampling across the entire model space mitigated uncertainty in high-temperature kinetic parameters, allowing us to predict a range of growth rates and morphologies for the SiC layer. The model accounts for parameter uncertainty stemming from limited experimental knowledge and successfully predicts relevant morphologies for the system. Experimental results validated the kinetic parameters of the simulations, offering valuable insights and potential constraints on the reaction kinetics. We further explored the significance of multi-phase-field model parameters on two key outputs, and found that the diffusion coefficient of liquid Si emerges as the most crucial parameter significantly impacting the SiC average layer thickness and grain count over time. This study provides valuable insights into the microstructure evolution of the Si-C binary system, offering pertinent information for the engineering of CMCs in industrial applications.

==> results.tex <==
%%
\section{Results and Discussion}\label{sec:results}
\par Our simulations examine the effects of diffusivities, interfacial energies, and mobilities on SiC growth at an isothermal temperature of 1450$^\circ$C. We explored the morphology and rate of growth of the SiC layer by querying different combinations of the kinetic parameters as listed in Table~\ref{tab:Kinetics}. The simulations begin post-nucleation when a continuous SiC layer has already covered the C substrate. The composition of the three phases is set to equilibrium values using the Si-C phase diagram. As the simulation begins, the SiC layer consumes Si and C phases to promote SiC growth until it reaches the top of the simulation domain. The simulations account for three major diffusion pathways: bulk diffusion, interfacial diffusion, and grain boundary diffusion, and we aim to understand the dominant kinetics.

\par Figure~\ref{fig:AvgThick} provides a summary of two extracted quantities, namely the area fraction and average thickness of the SiC layer, over time from 10,000 simulations. The solid red/blue lines represent the upper and lower limits of these quantities, while the results from other simulations are depicted within the gray-colored area. In these simulations, the SiC layer experiences growth for approximately 250 minutes. The phase-field method predicts a parabolic growth for the area fraction of the SiC layer and a linear growth trend for thickness evolution. The black markers with error bars correspond to our experimental measurements at different annealing times (20, 40, 60, and 90 minutes).

The reactive melt infiltration experiments on graphite preforms with Si were isothermal, maintaining a temperature of 1450$^\circ$C for durations ranging from 2 minutes to 4 hours. SiC layer formation was investigated using a diffusion couple configuration. The samples, infiltrated at various times, were characterized by SEM to measure SiC growth. At 20 minutes, the initial SiC layer thickness slightly deviates from the simulation's initial setting, bearing implications for optimizing kinetic parameters based on experimental observations. %Nonetheless, our focus is on growth rate and morphology rather than parameter optimization in this study.

\begin{figure*}[!ht]
    \centering
    \subfloat[]{\includegraphics[width=0.48\textwidth]{SiC5_areavstime2.png}}
    \subfloat[]{\includegraphics[width=0.48\textwidth]{2022-08-31-MaxMinSim5 (timeedit) (1).png}}
    \caption{Graphs for the growth of the SiC layer over time in 10,000 simulations. (a) Change of the area fraction of the SiC layer in time, (b) Change of the average thickness of the SiC layer in time. The upper and lower bounds in the simulations are shown in red and blue colored solid line and the intermediate calculations are shown in gray color. The experimental thickness and associated error bars from repeating the experiments are shown for thickness evaluations.}
    \label{fig:AvgThick}
\end{figure*}

\par We then analyze individual simulations or simulation groups, strategically identifying trends that may exist due to specific sets of parameters. In 5000 simulations, we systematically compared simulation groupings. This process provides crucial insights that direct the deliberate adjustment of parameter boundaries, bringing simulations closer to experimental outcomes. Furthermore, a detailed examination of simulation snapshots at various time markers provides insight into the kinetics, enabling a direct comparison of simulation thickness with experimental thickness. These snapshots serve as invaluable glimpses into the dynamics of phase evolution. We carefully interpret the kinetics, pinpointing the parameters exerting the most significant influence on simulation evolution. An illustrative example involves the identification of simulations successfully traversing multiple experimental points. By examining initial parameter conditions and iteratively refining constraints, we found simulation cases that align with an increasing number of experimental points.

\par Figure~\ref{fig:AreaFraction} displays the outcome of an individual simulation, specifically the area fraction of the SiC layer. SEM images capturing the evolution of the SiC layer at different time intervals accompany this simulation result. The corresponding thickness result is presented in the top-left corner of the figure. The marker points represent extracted area fraction values for this simulation, and a solid line is obtained through exponential curve fitting (i.e., $y = ae^{bx} + c$). The functional form of this fit is outlined below: 

%, along with the fitted constants for Figure~\ref{fig:AreaFraction}, Figure~\ref{fig:evolution}C, and Figure~\ref{fig:evolution}D, is outlined below:

\begin{equation}
    A_f=-1.678e^{-06}(e^{-.0006815t}) + 8.771e^{-07}
\end{equation}

%\begin{equation}
%    A_f=-7.461e^{-07}(e^{-.00131x})+8.824e^{-07}
%\end{equation}

%\begin{equation}
%    A_f=-1.877e^{-06}(e^{-.00089x})+7.761e^{-07}
%\end{equation}

\par Figure~\ref{fig:AreaFraction} illustrates that the thickness of the SiC layer shows a linear progression over the simulation time. The blue line denotes the maximum thickness measured at each point along the line. Notably, the maximum thickness exhibits less variability compared to experimental instances. Additionally, our simulation thickness trend generally appears steeper than that observed in experimental results. This discrepancy could stem from continuous nucleation in experiments, while our simulations exclusively involve coarsening in the phase field model. Another possible factor is that the interface may not be fully resolved with the presence of SiC, leaving empty areas where nucleation can persist, accentuating the thickness difference in simulations. This effort established a range for kinetic parameters and presented existing uncertainties in defining a realistic description of the reactive melt infiltration process. 

\begin{figure*}[!ht]
    \centering
    \begin{overpic}[width=0.99\textwidth]{C-Area_fraction3.png}%
%    \put(80,60){$A_f=a.e^{bx} + c$}%
    \scriptsize\put(55,60){$A_f=-1.67e^{-06}(e^{-0.000681t}) + 8.77e^{-7}$}%
%    y = -1.678204e-6*exp(-.00068154439*x)+8.771829e-07
    \end{overpic}
    \caption{Area fraction of SiC layer as a function of time from a phase-field simulation. An inlay of the thickness of this layer over time is also shown in the top left corner of the graph. The experimental SEM micrographs are embedded in this graph and show the growth of the SiC layer.}
    \label{fig:AreaFraction}
\end{figure*}

\par Figures~\ref{fig:evolution}(a) and \ref{fig:evolution}(b) present two instances of SiC layer evolution over time in our simulations, contrasting planar morphological evolution with scallop-like evolution. The color map illustrates the SiC phase-field order parameter profile. Simulation case I, depicted in Figure\ref{fig:evolution}(a), exhibits more grain coalescence. In contrast, simulation case II displays less coalescence but a planar growth. The persistence of smaller grains affects the larger grains that grow around them as SiC extends to the top of the simulation domain, resulting in columnar grain growth due to rapid grain boundary diffusion and lower interface energy between the liquid and SiC. On the other hand, scallop-type grains in simulation case II suggest the possibility of SiC grains dissolving rather than growing completely. The combination of certain parameters allows for either type of growth. Notably, there is minimal planar grain growth observed in our experimental results, indicating that while simulations can initiate planar growth, it may not be feasible experimentally. A comparison of simulation parameters in Table~\ref{tab:pars_two_sims} reveals that the most significant difference lies in the variation of interfacial energies. This underscores that grain boundary and liquid interfacial energies are the key parameters influencing the evolution of the simulations, while diffusivities and mobilities, with similar values, play a relatively minor role in driving these changes.

\par Figures~\ref{fig:evolution}(c) and \ref{fig:evolution}(d) correspond to the simulations that produced the SiC layer evolutions shown in Figures~\ref{fig:evolution}(a) and \ref{fig:evolution}(b). Both figures depict the growth of area fraction over time, along with the evolution of thickness in the upper left-hand corner. As mentioned earlier, the data is fitted to an exponential curve, and equations are provided in these figures. Additionally, simulation evolution images are included to visually represent the progress over time.

%%%%%%%%%%
\begin{figure*}[!ht]
    \centering
    \begin{overpic}[width=0.99\textwidth]{Two evolutions.png}%
    \put(0,61){(a)}%
    \put(0,30){(b)}%
    \end{overpic}
    \begin{overpic}[width=0.99\textwidth]{PR-2 Evolutions-area.png}%
    \put(45,29){(c)}%
    \tiny\put(25,5){$A_f=-7.461e^{-07}(e^{-.00131x})+8.824e^{-07}$}%
    \put(95,29){\normalsize{(d)}}%
    \tiny\put(72,5){$A_f=-1.877e^{-06}(e^{-.00089x})+7.761e^{-07}$}%
    \end{overpic}
    \caption{(a) and (b) Morphological evolution of the SiC layer during reactive melt infiltration at T = 1450$^{\circ}$C for two sets of kinetic parameters shown in Table~\ref{tab:pars_two_sims}. (c) and (d) The area faction of the SiC layer with the thickness curve embedded in the top left corner of each graph of these simulations.}
    \label{fig:evolution}
\end{figure*}
%%%%%%%%%%

\par The post-nucleation initial condition in our simulations imposes limitations related to dissolution or reprecipitation stages of SiC growth. We assume the nucleation stage is "complete" with the formation of a continuous SiC layer at the time we initiate our simulations, and the reaction transitions to being governed by diffusion. It is conceivable that there is a point in the experiment when the SiC layer becomes so thick that C diffusion essentially ceases, indicating a complete reaction in the diffusion-controlled regime. However, in both the conducted experiments and completed simulations, this point was not reached within the specified time frames.

%\textcolor{red}{We also debated analyzing the growth kinetics by application of the Johnson-Mehl-Avrami-Kolmogorov (JMAK) model~\cite{kolmogorov_andrei_nikolaevitch_study_1937, avrami_kinetics_1939, avrami_kinetics_1940, avrami_granulation_1941, william_a_johnson_reaction_1939}. The JMAK model is based on the extent of transformation achieved at any point in an isothermal phase transformation that proceeds through nucleation and growth. Because this type of growth only dominates up until the point where the SiC product layer becomes continuous, experimentally, this model is only applied up through approximately 18.5 minute reaction duration; the final experimental point before the SiC layer is observed to be continuous.}

\begin{table*}[!ht]
    \centering
    \begin{center}
    \begin{tabular}{ c c c c } 
     \toprule
     \multirow{2}{*}{Parameter} & Case I & Case II & \multirow{2}{*}{Unit} \\
     
           & \includegraphics[width=0.1\textwidth]{case1.jpg} & \includegraphics[width=0.1\textwidth]{case2.jpg} & \\
     \hline
     $D_L$ & $5.40\times10^{-13}$ & $2.97\times10^{-13}$ & $cm^2$/s\\
     $D_S$ & $3.21\times10^{-19}$ & $3.81\times10^{-19}$ & $cm^2$/s\\
     $D_I$ & $2.91\times10^{-18}$ & $6.62\times10^{-19}$ & $cm^2$/s\\
     $D_{IIS}$ & $8.42\times10^{-16}$ & $4.04\times10^{-16}$ & $cm^2$/s\\
     $D_{IIL}$ & $3.40\times10^{-15}$ & $3.01\times10^{-15}$ & $cm^2$/s\\
     $D_{GB}$ & $6.10\times10^{-15}$ & $7.30\times10^{-15}$ & $cm^2$/s\\
     $\sigma_S$ & 0.69 & 0.61 & J/$m^2$\\
     $\sigma_{GB}$ & 0.37 & 0.29 & J/$m^2$\\
     $\sigma_L$ & 0.26 & 0.11 & J/$m^2$\\
     $M_S$ & $9.34\times10^{-08}$ & $9.37\times10^{-08}$ & $m^3/{J.s}$\\
     $M_L$ & $5.76\times10^{-07}$ & $4.52\times10^{-07}$ & $m^3/{J.s}$\\  
     \bottomrule
    \end{tabular}
    \end{center}
    \caption {Parameters with their associated values for the completed simulations in Figure \ref{fig:evolution}. Note, parameters are defined in Table ~\ref{tab:Kinetics}.} \label{tab:pars_two_sims}   
\end{table*}

%% feature importance study
\par We further explored the significance of multi-phase-field model parameters on two key outputs: the average thickness of the SiC layer at a fixed time (Output I) and the grain count in the confined simulation domain after a specific fixed time (Output II). We employed both model-agnostic and model-dependent approaches for feature importance analysis, utilizing Lasso linear regression and permutation feature importance methods. The outcomes depicted in Fig.~\ref{fig:ML_feature_importance} affirm that both machine learning methods identify the same features as the most influential ones for Outputs I and II. Specifically, the diffusion coefficient of liquid Si emerges as the most crucial feature significantly impacting the SiC average layer thickness and grain count over time. Other liquid parameters, such as liquid Si/SiC interface mobility and liquid/SiC interface diffusivity, also hold substantial importance, although the degree of significance may vary depending on the method employed (i.e., Lasso or permutation methods).

\par Regarding SiC layer thickness (Output I), the four most influential model parameters, identified through the permutation by random forest regression ML method, include liquid Si diffusion, Si/SiC interface diffusivity, Si/SiC interface energy, and solid C diffusion. Notably, the first influential parameter is consistent between the two methods. However, the Lasso model diverges slightly, listing Si diffusion, Si/SiC interface mobility, Si/SiC interface energy, and Si/SiC interface diffusivity as the most influential parameters, aligning closely with the permutation method. For grain count (Output II), the four most influential model parameters are liquid Si diffusion, Si/SiC interface diffusivity, SiC/SiC interface energy, and Si/SiC interface energy. Both ML methods precisely agree in this case, and the ranking obtained is consistent for the first five parameters.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1\textwidth]{Fig7_NEW.png}
    \caption{Multi-phase-field model feature importance study for the SiC layer growth (output I) and the SiC grain coalescence (output II). Lasso model coefficient regularization and Random Forest permutation predict a similar rank of importance for liquid diffusion, liquid interface mobility, grain boundary interface energy, and liquid/IMC interface energy for grain count model output. Likewise, these models predict a similar rank of importance for liquid diffusion, liquid/IMC interface diffusion, liquid mobility, and grain boundary interface energy for IMC thickness model output.}
    \label{fig:ML_feature_importance}
\end{figure*}


\section{Conclusions}\label{sec:conc}


\par Our developed multi-phase-field model offers insights into the kinetics of SiC growth during the reactive melt infiltration process at 1450 $^{\circ}$C. By considering the uncertainty in model parameters arising from limited experimental knowledge in the Si/C system, we explore various SiC morphologies, aligning with concurrent experimental observations. Beyond visualizing the evolving SiC microstructure, our model provides valuable information on energy terms related to grain boundaries and interfaces. This data enables further exploration of the relationship between grain boundary diffusion rates, bulk diffusion, and SiC growth at the interface. Our observations highlight the growth of SiC over the graphite substrate, providing insight on the extent of the kinetic parameters in Si-C system. This investigation serves as a crucial tool for understanding processes at extremely high temperatures, where instrumentation limitations hinder direct kinetic measurements. For experimental validation, we create carbon and SiC powder-based preforms and infiltrate them at different time frames, enabling a comparison between simulated SiC growth and experimental samples. The resulting data not only provides computational values for diffusivities, interfacial energies, and mobilities but also furnishes experimental insights into the kinetics of the reaction. The study demonstrates the qualitative reproduction of experimental results regarding the grain growth of SiC over time. Computational investigation of SiC growth during reactive melt infiltration process proves considerably more intricate than observations from experimental work. SiC grain growth emerges as an 11-dimensional problem with limited quantitative guidance available.

\par The results are proof of the application of the phase field model on the prediction of the microstructure evolution in the Si-C binary system. Both experiments and calculations show similar growth over time. The developed model does have several limitations, including the need to conduct simulations post-nucleation to observe a full picture of SiC evolution. Future refinement of our model will include nucleation to enable the observation of SiC growth from the earliest stages of the melt infiltration process.

\par Our focus extends to identifying strategies for controlling microstructure evolution to align with experimental growth, laying the groundwork for future applications. This knowledge holds promise for ternary systems, offering valuable insights into the utility of this information for other ceramic matrix composites (CMC) processed through reactive melt infiltration. Specifically, applications involving Si-Hf-C or Si-Zr-C systems stand to benefit significantly. Simulations that elucidate the structural evolution in CMC systems contribute to the identification of materials with advantageous properties, holding implications for aerospace, aviation, and nuclear applications.

\section{Appendix}
\par Listed below are the parameters of the energy functions from the SGTE database and others used to obtain energy curves shown in Fig.~\ref{fig:Free_Energy} (equations 9-11). 

\footnotesize

\begin{table*}[!ht]
    \centering
    \small
    \begin{adjustbox}{width=\textwidth,center}
    \begin{tabular}{llc} \toprule
       Parameter & & Reference \\ \midrule
       $G^{Graphite}_C$ & $-17368.441+170.73 \cdot T-24.3 \cdot T \cdot \text{ln(T)}-0.4723E{-3} \cdot T^{2}+2562600 \cdot T^{-1}-264300000 \cdot T^{-2}+1.2E10 \cdot T^{-3}$+Gpres & ~\cite{du1999experimental}
       \\
       $G^{Liq}_C$ & $100000.559+146.1 \cdot T-24.3 \cdot T \cdot \text{ln(T)}-0.4723E{-3} \cdot T^{2}+2562600 \cdot T^{-1}-2.643E{8} \cdot T^{-2} + 1.2E10 \cdot T^{-3}$+Gpres & ~\cite{du1999experimental}
       \\
       $G_{SiC}$ & $-44291.98+135.5731 \cdot T-20.63973 \cdot T \cdot \text{ln(T)}-2.15133E{-3} \cdot T^{2}+4E{5} \cdot T^{-1}+10^{7} \cdot T^{3}$ & ~\cite{du1999experimental}
       \\
       $G^{SER}_{Si}$ & $-9457.642+167.281367 \cdot T-27.196 \cdot T \cdot \text{ln(T)}-420.369E{28} \cdot T^{-9}$ & ~\cite{dinsdale_sgte_1991}
       \\
       $^0L^{Liq}_{ij}$ & $+25644.97-6.38115 \cdot T$ & ~\cite{cupid_thermodynamic_2007} \\
       GHSERSI & $-7.04\times10^{4}$ \\
       GSOLC & $-3.5202\times10^{4}$ \\
       GLIQC &  $3.97\times10^{4}$ \\
       GLIQSI & $-7.15\times10^{4}$ \\
       GSOLSI & $-7.04\times10^{4}$ \\
       GSIC & $-1.63\times10^{5}$ \\
       GCG & $-3.52\times10^{4}$ \\
       GDIAC & $-2.58\times10^{4}$ \\
       GHSERC & $-3.52\times10^{4}$
       \\ \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Thermodynamic parameters used for the calculation of energy curves involved in SiC reactions.}
    \label{tab:my_label}
\end{table*}

\section{Acknowledgement}
\par The authors would like to acknowledge the support from AFRL through sub-contract 165852-19F5830-19-02-C1. MM and EJMIII acknowledge support from the National Science Foundation, grant No. 1545403, Data-Enabled Discovery and Design of Energy Materials, D3EM.  

\label{S:6}
